The influence of color on prices of abstract paintings

Determination of price of an artwork is a fundamental problem in cultural economics. In this work we investigate what impact visual characteristics of a painting have on its price. We construct a number of visual features measuring complexity of the painting, its points of interest, segmentation-based features, local color features, and features based on Itten and Kandinsky theories, and utilize mixed-effects model to study impact of these features on the painting price. We analyze the influence of the color on the example of the most complex art style - abstractionism, by created Kandinsky, for which the color is the primary basis. We use Itten's theory - the most recognized color theory in art history, from which the largest number of subtheories was born. For this day it is taken as the base for teaching artists. We utilize novel dataset of 3885 paintings collected from Christie's and Sotheby's and find that color harmony has some explanatory power, color complexity metrics are insignificant and color diversity explains price well.

==> results_OLS.tex <==
\begin{tabular}{ll}
\toprule
{} &         Coef. \\
\midrule
const                &  (11.5777)*** \\
square\_m             &   (0.7039)*** \\
ExhibitedNum         &   (0.2385)*** \\
ProvenanceNum        &   (0.3108)*** \\
LiteratureNum        &   (0.2223)*** \\
oil                  &   (0.6982)*** \\
ink                  &   (0.1635)*** \\
lithograph           &  (-0.4921)*** \\
canvas               &   (0.3234)*** \\
contrast\_h           &   (0.1404)*** \\
area\_of\_fls          &   (0.2029)*** \\
number\_of\_segments   &    (0.246)*** \\
date\_of\_birth        &   (0.1296)*** \\
gouache              &    (0.1026)** \\
X\_comp               &   (-0.0793)** \\
area\_of\_sls          &    (0.0822)** \\
ccm                  &   (-0.2103)** \\
contrast\_v           &   (-0.1095)** \\
contrast\_s           &    (0.1106)** \\
paper                &   (-0.1226)** \\
turquoise            &     (0.0636)* \\
blue                &     (0.0969)* \\
mean\_h               &     (0.0977)* \\
mean\_v               &    (-0.1063)* \\
Sign                 &    (-0.0475)* \\
\bottomrule
\end{tabular}


==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


